Covariate Distribution Aware Meta-learning

Meta-learning has proven to be successful for few-shot learning across the regression, classification, and reinforcement learning paradigms. Recent approaches have adopted Bayesian interpretations to improve gradient-based meta-learners by quantifying the uncertainty of the post-adaptation estimates. Most of these works almost completely ignore the latent relationship between the covariate distribution $(p(x))$ of a task and the corresponding conditional distribution $p(y|x)$. In this paper, we identify the need to explicitly model the meta-distribution over the task covariates in a hierarchical Bayesian framework. We begin by introducing a graphical model that leverages the samples from the marginal $p(x)$ to better infer the posterior over the optimal parameters of the conditional distribution $(p(y|x))$ for each task. Based on this model we propose a computationally feasible meta-learning algorithm by introducing meaningful relaxations in our final objective. We demonstrate the gains of our algorithm over initialization based meta-learning baselines on popular classification benchmarks. Finally, to understand the potential benefit of modeling task covariates we further evaluate our method on a synthetic regression dataset.

==> commands.tex <==
\newcommand*{\thead}[1]{%
\multicolumn{1}{c}{\bfseries\begin{tabular}{@{}c@{}}#1\end{tabular}}}

\def\V#1{\mathbf{#1}}
\def\C#1{\mathcal{#1}}
\def\R#1{\mathrm{#1}}
\def\B#1{\mathrm{#1}}

\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0,0.7,0}
\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{0.6,0,0}
\definecolor{Orange}{rgb}{1,0.5,0}


\newcommand{\am}[1]{\textcolor{Blue}{[#1 --Amrith]}}
\newcommand{\sd}[1]{\textcolor{Green}{[#1 --Saket]}}

==> sections/abstract.tex <==
\begin{abstract}
    Meta-learning has proven to be successful at few-shot learning across the regression, classification and reinforcement learning paradigms. 
    Recent approaches have adopted Bayesian interpretations to improve gradient based meta-learners by quantifying the uncertainty of the post-adaptation estimates. Most of these works almost completely ignore the latent relationship between the covariate distribution $(p(x))$ of a task and the corresponding conditional distribution $p(y|x)$. In this paper, we identify the need to explicitly model the meta-distribution over the task covariates in a hierarchical Bayesian framework. We begin by introducing a graphical model that explicitly leverages very few samples drawn from $p(x)$ to better infer the posterior over the optimal parameters of the conditional distribution $(p(y|x))$ for each task. Based on this model we provide an inference strategy and a corresponding meta-algorithm that explicitly accounts for the meta-distribution over task covariates. Finally, we demonstrate the significant gains of our proposed algorithm on a synthetic regression dataset.  
\end{abstract}

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Cognizant of the fact that the generalization performance of few-shot algorithms depends on a varying number of factors ranging from sample size, hypothesis class complexity to the optimization algorithm, input distribution; in this work we focus our efforts on improving meta-learning algorithms by using the covariate distribution to infer the adapted parameters via a principled Bayesian approach. We begin by deriving \textsc{elbo} bounds for the hierarchical Bayes formulation and follow it up with a meta-learning algorithm to infer the posterior over the network parameters. Finally, we show some preliminary results on a synthetic regression dataset designed to test the usefulness of our method.

Motivated by the empirical gains observed, we plan to extend our work to more challenging few-shot image classification benchmarks like mini-imagenet \cite{ravi2016optimization} and FC100 \cite{oreshkin2018tadam}. We also acknowledge that the proposed framework warrants a more rigorous theoretical analysis to understand exactly how inferring the covariate distribution can impact regret bounds  \cite{khodak2019adaptive, khodak2019provable}  in the online few-shot setting or even generalization error bounds in the classical one.

==> sections/experiments.tex <==
\section{Experiments and Results}
\label{sec:experiments}

% \am{describe setup -- dataset creation -- baselines  -- finally of our table}

In order to first litmus test our approach on a simpler task we begin by evaluating it on a synthetic regression dataset borrowed from \citet{vuorio2019multimodal} and defer further experimentation on more complicated real world datasets to future work. Most meta-learning algorithms have been tested on regression datasets where the covariate distribution is same across all tasks. We thus describe how we suitably modify the original dataset so that there exists a structure over the set of covariate distributions across tasks. This enables us to fairly evaluate our method against the baselines in the proposed setting.

We compare our algorithm with the popular gradient based meta-learning approach \textsc{maml} introduced by \citet{finn2017model}. Additionally, we also chose as baselines Amortized \textsc{maml} \cite{ravi2018amortized} and \textsc{m-maml} \cite{vuorio2019multimodal} which are exemplars of the Bayesian and task-specific initialization type approaches respectively. These methods either model the task-parameters as Bayesian random variables (former) or adapt the parameters of the optimizer based on the input dataset (latter) and hence warrant a close comparison with our proposed methodology. 


\begin{table}[!ht]
    \centering
    \begin{tabular}{c c c c}
    \textbf{Model}     & \textit{sine}  & \textit{sine-quad-linear} & \textit{five} \\\toprule
    \textsc{maml} & 0.05 & 1.27  & 1.69   \\
    Amortized \textsc{maml} & 0.07 & 1.39  & 1.13   \\
    \textsc{m-maml} &  0.04 & 0.59  & 0.93\\
    Ours  & \textbf{0.008} & \textbf{0.39} & \textbf{0.89}\\
    \end{tabular}
    \vspace{0.5em}
    \caption{Comparison of post adaptation test performance (\textsc{mse} loss) on three regression datasets when the true hypothesis class depends on the covariate distribution.}
   \label{tab:results-1}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{c c c c}
    \textbf{Model}     & \textit{sine}  & \textit{sine-quad-linear} & \textit{five} \\\toprule
    \textsc{maml} & 0.04 & 1.15  & 1.73   \\
    Amortized \textsc{maml} & 0.07 & 1.41  & 1.08   \\
    \textsc{m-maml} &  \textbf{0.03} & 0.51  & 0.88\\
    Ours  & 0.04 & \textbf{0.51} & \textbf{0.84}\\
    \end{tabular}
    \vspace{0.5em}
    \caption{Comparison of post adaptation test performance (\textsc{mse} loss) on three regression datasets when the true hypothesis class is independent of the covariate distribution.}
    \label{tab:results-2}
\end{table}


    


\paragraph{Dataset} The covariate distribution for each task $\C{T}$ is given by a normal $\C{N}(\mu_\C{T}, \sigma_{\C{T}})$ whose parameters are sampled from a discrete distribution over $P$ pairs $\{(\mu_p, \sigma_p)\}_{p=1}^{P}$. The pairs $p_1, \dots p_P$ are fixed in the beginning once they are sampled from a pair of independent uniform priors, $p_i \sim (\C{U}(-10, 10), \; \C{U}(0, 10))$. The parameters of the discrete distribution are sampled from a Dirichlet prior $(\textrm{Dir}(\alpha_p=1))$.  Following \cite{vuorio2019multimodal}, the optimal hypothesis for each task is sampled from one of many modalities or hypothesis classes. The hypothesis classes considered are : \textit{sine}, \textit{linear}, \textit{quad}, \textit{transformed-L$_1$} and \textit{tanh}. For each task, having chosen a hypothesis class, the parameters of the optimal hypothesis (like slope of a linear functions) is chosen based on uniform distributions over the following \footnote{Taken as is from \cite{vuorio2019multimodal}. Re-iterated for the sake of completion.}: 
\setlist{nolistsep}
\begin{enumerate}
    \item \textit{sine}: $f(x)=A\cdot(sin (w \cdot x) + b)$, with $A \in [0.1, 5.0], w \in [0.5, 2.0]$ and $b \in [0, 2\pi]$.
    \item \textit{quad}: $f(x)=A\cdot(x - c)^2 + b$ with 
 $A \in [-0.15, -0.02] \cup [0.02, 0.15], c \in [-3.0, 3.0]$ and $b \in [-3.0, 3.0]$.
    \item \textit{linear}: $f(x) = A \cdot x + b$, $A \in [-3, 3], b \in [-3, 3]$.
    \item \textit{transformed-L$_1$}: $f(x)=A \cdot |x - c| + b$, with $A \in [-0.15, -0.02] \cup [0.02, 0.15], c \in [-3.0, 3.0]$ and $b \in [-3.0, 3.0]$.
    \item \textit{tanh}: $f(x) = A \cdot tanh(x-c)+b$ with $A \in [-3.0, 3.0], c \in [-3.0, 3.0], b \in [-3.0, 3.0]$.
\end{enumerate}
For each of the true hypothesis classes above the final value of $\V{y}^{(i)}_j$ is generated by adding an independent error term $\epsilon$ sampled from a normal distribution with mean $0$ and standard deviation of $0.3$ \textit{i.e} $\V{y}_j^{(i)} = f(\V{x}_j^{(i)}) + \epsilon$. 

We consider two cases, \textit{first} where there exists a relation between the parameters (mean, variance) of the covariate distribution and the optimal hypothesis class chosen for a task and \textit{second} when the optimal hypothesis class is chosen independent of the mean, variance of the covariate distribution. We highlight the results in each case separately.

% , five pairs $\{\V{x}_j, \V{y}_j\}_{j=1}^{5}$ are sampled using three-step process: 
% \begin{enumerate}[(i)]
%     \item sample We experiment with three datasets \textit{sine}, \textit{sine-quad-linear} and 
% \end{enumerate}

% \textit{five} where



\paragraph{Case-I: With a specific relation} This setting conforms to the case when $z_y {\not\!\perp\!\!\!\perp} z_x | \theta$ in Fig.~\ref{fig:gm_CPMAML}. We experiment with three different meta-distributions which are of different complexities owing to the variety (number) of hypothesis classes each of them span. The datasets are listed as follows:
\setlist{nolistsep}
\begin{enumerate}
    \item \textit{sine}: true hypothesis for each class is given by a sinusoidal function with parameters sampled from distributions mentioned previously. The range for each of the parameters is split into $P=3$ disjoint sets, each one corresponding to a specific covariate distribution. 
    \item \textit{sine-quad-linear}: each of the three hypothesis classes are mapped to a specific covariate distribution. Thus, once the parameters of the covariate distribution are sampled based on the discrete prior, the corresponding hypothesis class is also chosen and a task is sampled from it.
    \item \textit{five}: similar to the previous case with the distinction that all five hypothesis classes are considered in this dataset \textit{i.e} $P=5$.
\end{enumerate}
% consist of varying complexoties 

Table~\ref{tab:results-1} highlights the Mean Squared Errors (\textsc{mse}) achieved by our method and the baselines on the three regression datasets described above. We can see that when there exists a relation between the true hypothesis class and the covariate distribution our approach performs significantly better than other state-of-the-art approaches for regression. Interestingly, improvements are also observed for the \textit{five} dataset which was specifically introduced by \citet{vuorio2019multimodal} for evaluating \textsc{m-maml}. The Bayesian model Amortized \textsc{maml} performs poorly since unlike our approach it fails to acknowledge the latent relationship between the covariate distribution and the posterior over the five hypothesis classes. 
% in cases when the task distribution is more complex, spanning a wider array of hypothesis classes (\textit{five} dataset).


% \label{subsec:case-II}
\paragraph{Case-II: Independent} This setting conforms to the case when $z_y \perp\!\!\!\perp z_x | \theta$ in Fig.~\ref{fig:gm_CPMAML}. In Table~\ref{tab:results-2} we demonstrate that the performance of our approach is no worse (if not better) than other methods which assume the independence by default. Once again we experiment with the same three types of meta-distribution mentioned in the previous case. 
% We also observe some gains for the \textit{five} dataset where the reduction is \textsc{mse} loss is 



\paragraph{Implementation} The conditional $p(y|x)$ is modeled using a three-layered neural network with hidden sizes $100, 100, 100$. The networks $\gamma_\mu(\cdot; \beta), \gamma_\sigma(\cdot; \beta)$ which take as input the sequence of labeled samples in a dataset $\C{D}_i^S$ are modeled using a common Recurrent Neural Network \textsc{rnn} backbone with output of dimension $28$. This can be referred to as the \textit{task-embedding} \cite{vuorio2019multimodal}. 
The mapping of task-embedding to $\lambda_i^{(0)}$, given by $f_\beta(\cdot)$ is modeled similar to \textsc{m-maml} as well as the modulation over $\lambda_i^{(0)}$ which gives us the final initialization of the network parameters \footnote{The code for our implementation was in part borrowed from \tiny{\url{https://github.com/vuoristo/MMAML-Regression}}}. Following prior work \cite{finn2017meta}, a bias-transformation of size $20$ was appended to the inputs. 
% Also, the final initialization of the network parameters is given by a simple modulation of $\lambda^0_i$. 
% For more details, we refer the reader to \citet{vuorio2019multimodal}.
% given by the neural network to modulate meta-learned initialization. 
% \am{Have a paragraph on implementation details.}
The total number of training tasks used were $10,000$ with $m'=m-m'=5$ samples for the support and query sets for each task. Adam optimizer with an initial learning rate of $0.001$ was used to train the meta-learner. Additionally, all \textsc{kl} terms were re-weighted with a weight of $0.01$. 

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% \am{mention somewhere that if we have additional unlabeled examples, the benefits of our method amplify. }
% \sd{introduction/motiv to meta-learning}
Learning quickly or with very few samples has been a long-term goal of the machine learning community. The field of meta-learning has recently made significant strides towards achieving that goal. Meta-learning \cite{nichol2018first, ravi2016optimization, finn2017model} comprises of a set of algorithms designed to exploit prior experiences from multiple tasks (drawn from a task distribution) for improving sample-efficiency on a new but related task from the same distribution. Given the increasing cost of getting annotated samples on an ever-increasing variety of related tasks, the practical scope of these algorithms is immense.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/example.png}
    \caption{Samples of tasks drawn from a meta-distribution categorized based on its corresponding hypothesis class. The red crosses indicate the labeled sampled points and the blue, green dashed lines represent the true hypothesis for two different tasks from the same class. We can clearly see that the hypothesis class is not independent of the task specific input distribution $p(x)$. For example, the covariate distribution for \textit{sinusoidal} tasks have a higher support in the negative region (in $\B{R}$) where as the support is confined to a much narrower positive region for \textit{linear} tasks.\vspace{-2.1em}
}
    \label{fig:example}
\end{figure}

% \sd{introduction/motiv to Gradient based ML, MAML, Bayesian MAML}
Most meta-learning methods can be classified into two broad categories (i) \textit{gradient-based} \cite{ravi2018amortized, denevi2019learning, finn2017model} approaches that meta-learn parameters of optimization algorithms (like initialization and learning rate) in a way that the meta-learner (optimizer) is amenable to quickly adapt on a new task by performing gradient descent on a very small number of labeled samples, and (ii) \textit{amortized-inference} \cite{snell2017prototypical, lee2019meta, bertinetto2018meta} based approaches that directly infer the optimal parameters of a new task without performing any gradient based optimization. 
In general, such algorithms learn to adapt the parameters of a complex neural network using only a few samples from an unseen task in a way that the \textit{adapted network} generalizes well \cite{wang2019generalizing}.
In this work, although we focus on improving gradient-based methods, we believe that our core idea can be adapted to the latter as well. 
% Deep learning models learn through backpropogation of gradients. Therefore, \cite{ravi2016optimization}, \cite{finn2017model}, \cite{nichol2018first} defines an intuitive way to learn fast by developing optimization based meta-learning methods are designed to cope with a small number of training samples, or to converge within a small number of optimization steps. 
% \cite{finn2017model} proposes a model agnostic framework MAML that searches for good initializations for model parameters that can quickly adapt to a new task using a few steps of gradient descent. More generally, 
Recent works \cite{finn2018probabilistic}, \cite{ravi2018amortized}, \cite{kim2018bayesian} have used a Bayesian framework to learn a suitable prior over the network parameters by leveraging the inherent structure of the task distribution. 
% The Bayesian approach specifically aids in modelling the uncertainty \cite{gal2016dropout} in the prediction of the optimal parameters on a new task. 
By viewing the parameters of a meta-learner through a Bayesian lens we can use the predictive posterior \cite{gal2016dropout} to estimate the uncertainty of the adapted parameters for each task \cite{ravi2018amortized}.



In a Bayesian meta-learner \cite{kim2018bayesian, finn2018probabilistic, ravi2018amortized}, the posterior over the adapted network parameters for a new task is typically inferred using a few samples from the task along with a meta-learned prior. In this work, we hypothesize that the covariate distribution of a task can also influence the posterior over the adapted network parameters. To the best of our knowledge none of the existing meta-learning algorithms like \citet{bertinetto2018meta, rajeswaran2019meta, ravi2018amortized, finn2018probabilistic} explicitly utilize the information present in the covariates to improve the estimate of the adapted parameters. 
This is done by modeling the latent factors of the covariate distribution.
We define a prior not only on the network parameters (which determine the conditional $p(y|x)$) but also on the covariate distribution $p(x)$. 
Our meta-learning objective involves maximizing the joint likelihood $p(x, y)$ as opposed to just $p(y|x)$ 
which leads to meta-parameters sharing information about the covariates across tasks, in addition to the optimal network parameters. 
This way the latent factors of the covariate distribution $p(x)$ of a new task can be quickly inferred from very few covariates. Finally, the inferred latent covariate factors are used to infer the posterior over the adapted network parameters.
% allowing us to use learned $p(x)$ to better estimate parameters for $p(y|x)$. 

% both observed variables x and y. 
% Finally, we define a meta-learning algorithm to concretely specify all the probability distributions and ways to efficiently optimize the above objective. 

% We do this by modeling the latent factors of the covariate distribution 
% first inferring the  the inferred random variables for the covariates using it to inform an initialization for the network parameters. Using covariates in a Bayesian model also helps us to theoretically reason about our model in a probabilistic framework which is not possible for \textsc{m-maml}


For simplicity, we motivate the need to model covariates via a synthetic example in Fig.~\ref{fig:example}. The meta-distribution consists of tasks with optimal hypothesis $h \in \C{H}$$=$$\bigcup \; \{\C{H}_s, \C{H}_l, \C{H}_t, \C{H}_q\}$ that can be classified into four hypothesis classes: \textit{sinusoidal} ($\C{H}_s$), \textit{linear} ($\C{H}_l$), \textit{tanh} ($\C{H}_t$) and \textit{quadratic} ($\C{H}_q$).
% follow a multi-modal distribution where the mode in which task lies depends on the $p(x)$ of that task. 
We note that the support of the input distribution is vastly different for each of the four hypothesis classes. Thus, intuitively we can see that inferring properties of the covariate distribution of a task can be helpful in adjusting the posterior over the network parameters. For example, for a given task if we only observe negative covariates in the range $[-10, -5]$ we can adapt the posterior to have a higher measure for $\C{H}_s$ (sinusoidal hypothesis).
% Therefore, the meta-distribution over the covariates of different tasks can better assist in learning the multi-modal prior over parameters of $p(y|x)$. Also, for a new task, we can identify the mode in which it lies by using just the input $p(x)$ of this task. 
% \sd{cite things in this intuition?}

We can generalize the above intuition to real-world meta-learning problems as well, especially for high-dimensional data like images. 
Particularly, in the limited availability of labeled data, semi-supervised methods \cite{chapelle2009semi} tend to leverage unlabeled data (and hence covariate distribution) to attain generalizable models \cite{berthelot2019mixmatch}
On similar lines, modeling the meta-distribution over the covariates can help inferring the task-specific covariate distribution which can then better inform task-specific features for image classification. 
In few-shot classification, images for different tasks can lie on different manifolds \cite{saul2003think} of varying complexities. Information about the covariates (by modeling the unlabeled data) can help us better estimate the required complexity of the discriminative features for a given task.
% In few-shot classification, images for different tasks can lie on different manifolds \cite{saul2003think} of varying complexities.
% Thus, the discriminative features needed to achieve good generalization performance given only a few samples is inherently dependent on the covariate distribution of the task.
% rendering its space to be dependent on the covariate distribution (manifold of images). 
% (since the manifold and the inherent complexity is a manifestation of the semantic concepts that the classes in a task represent).
For example, distinguishing species of plants can be considered harder than classifying mammals since the features of plant images may be cluttered on a low-dimensional manifold as opposed to the possibly well separated features in the case of mammals. 
% The inherent complexity of the task is a manifestation of the semantic concepts that the classes represent.
Thus the former may require having complex (non-linear) decision boundaries as opposed to simpler linear classifiers in the case of the latter. 
% Therefore, modeling a meta-distribution over covariates to inform the posterior over the optimal parameters of a new task can help us better estimate the required complexity of the discriminative features for that task.

The main contributions of our work are as follows: (1) we identify the need to model the latent structure present in the covariate distributions $(p(x))$ for a sequence of tasks (2) to the best of our knowledge we are the first to propose a Bayesian framework which exploits this latent information to better infer the posterior over the adapted network parameters  (that define $p(y|x)$) (3) we propose a gradient based model-agnostic meta-learning algorithm that is an instantiation of our probabilistic theory and demonstrate its benefits on synthetic regression datasets.  

% \sd{Brief idea of how can be tackled?}
% We extend the Bayesian framework to model the structure of covariate distribution of different tasks. In our framework, we define a prior on not only network parameters defining $p(y|x)$ but also on covariate distribution $p(x)$. We then define a novel meta-learning objective over task specific variational parameters and task-agnostic meta-parameters, by maximizing the likelihood for both observed variables x and y. This results in meta-parameters also sharing information about the covariates across tasks, and hence the variational parameters for p(x) of a new task can be quickly learned from very few samples, allowing us to use learned $p(x)$ to better estimate parameters for $p(y|x)$. Finally, we define a meta-learning algorithm to concretely specify all the probability distributions and ways to efficiently optimize the above objective. 

% \sd{, probab framework, 
% Taxonomy of our approach, compare and contrast to existing work}

\section{Related Work}
\label{sec:related-work}

% As per best of our knowledge, ours is the first work that explicitly models the covariate distribution in the meta-learning setting. 
Our methodology is complementary to most existing works in the probabilistic meta-learning literature. We borrow the basic hierarchical Bayes framework from \citet{ravi2018amortized, finn2018probabilistic} and extend it to model Bayesian variables that generate the covariate distribution for a task. This enables our method to be model-agnostic while having the ability to benefit from the latent relationship between the task covariates and the optimal parameters as mentioned in Sec.~\ref{sec:introduction}. 
In the non-Bayesian setting, the \textsc{m-maml} algorithm proposed by \citet{vuorio2019multimodal} is mildly similar to our approach in the sense that they learn task specific initializations instead of a single one as originally introduced by \citet{finn2017model}. \textsc{m-maml} uses the labeled samples to infer an initialization for a given task and hence one can view the covariate distribution as being used indirectly. 
% to run amortized inference for the initialization. 
But they fail to explicitly model the mutual information between the covariates and adapted parameters.  
% . They use task embedding to choose the task-specific initializations for the network.
% However, they fail to provide any intuitive background theory behind the significance of task-embedding. 
On the other hand, our approach is more direct since it \textit{first} infers the posterior over the latent factors of the covariate distribution via a maximum likelihood objective and then uses the inferred posterior to improve the adaptation of network parameters. Additionally, our framework is capable of modeling the uncertainty of the adaptation which can prove to be be critical in the few shot scenario.
% in case of less-interpretable task embeddings. 

% their idea by introducing task-specific prior which is based on tasks' covariate distribution rather than task-embedding. 

% \sd{List of contributions}





% ----------------
% \am{begin  by talking abt Meta-Learning in general, talk about its taxonomy a bit, then a bit about bayesian approaches. Identify where our approach fits in the taxonomy -- can also cite related works here (refer to amortized MAML and MMAML paper for good related works?)}

% \am{re-phrase motications from rel. work as needed.}

% \am{put a figure at the top right corner -- simple motivating example of why our approach may be helpful}. 

% \sd{introduction to the our approch, motivation of why,  contributions list refer amortized maml, 
% MMAML
% PMAML - think compare contrast
% Bayesian MAML - think compare contrast
% }

% \am{content from other overleaf -- rephrase and cut short as needed. they can be used in motivation part}

% \cite{finn2018probabilistic}, \cite{ravi2018amortized}, \cite{kim2018bayesian}
% defined the meta-learning framework in Bayesian setting to model the uncertainity in the predictions. Furthermore, each of them uses non-parametric variational inference technique to effectively learn complex uncertainity structures. They involve learning a prior over model parameters using the task distribution in order to quickly adapt them using a very few examples for a particular task. However, as per best of our knowledge, the previous works share the prior information in a limited setting by defining it over only $p(y|x)$ distribution rather than the joint of $p(x,y)$\\
% In our work, we propose to extend this setup to account for distribution of covariates. This is based on our hypothesize that information about meta-distribution over the covariate distribution influence the parameters chosen to model task-specific distribution $p(y|x)$. Further, we chose the probabilistic model as our base because not only it accounts for uncertainity in prediction, but also provides the flexibility to share prior learnt from meta-distribution to each of the tasks.\\

% We organise this section as follows. First in \ref{subsec:deriv}, we formally derive the variational form of our model to maximize the likelihood of data while being influenced by the induced priors. Next in \ref{subsec:algorithm}, we formally write the algorithm for meta-training and testing while also highlighting the key differences to existing work. In the end \ref{subsec:sskdl}, we show a case study for regression task by incorporating existing semi supervised method \cite{jean2018semi} into meta-learning framework.\\ 






==> sections/methodology.tex <==
\section{Methodology}
\label{sec:methodology}
% \am{start with some notations for meta-learning in general (task, query, support). then we can introduce the graphical model we are considering and its notations. then formal derivations and finally the proposed algorithm. in the end instantiate our approach with our specific model.}
% \am{Add figure with the Task embedding model -- and it also has notations}
We begin by introducing some notations for the meta-learning setup used in the rest of the paper followed by the proposed probabilistic framework which explicitly exploits (i) the structure of the covariate distributions across tasks (ii) the relation between the covariate distribution and optimal hypothesis for a given task. We then derive the Maximum Likelihood Estimation (\textsc{mle}) objectives for the observed variables in our model and show how the \textsc{mle} derivations can inform a novel meta-learning objective. Finally, we discuss a specific meta-learning algorithm that can efficiently optimize the proposed objective. We do this via an instantiation of the generic approach obtained by making certain simplifying assumptions in the original framework.



\textbf{Notations} We are given a sequence of $n$ tasks $\{\C{T}_i\}_{i=1}^{n}$ with each task $\C{T}_i$ having $m$ labeled samples given by the dataset $\C{D}_i = \{\V{x}_j^{(i)}, \V{y}_j^{(i)}\}_{j=1}^{m}$ where $\V{x}_j^{(i)} \in \C{X} \subset \B{R}^{k}$ and $\V{y}_j^{(i)} \in \C{Y}\,\, \subset \B{R}$. Following the definitions introduced by \citet{finn2018probabilistic} we split the dataset  $\C{D}_i := \{\C{D}_i^{S}, \C{D}_i^{Q}\}$ into support ($\C{D}^{S}_i$) and query $(\C{D}^{Q}_i)$ sets respectively with $|\C{D}_i^S|=m', |\C{D}_i^Q|=m-m'$. Each sample in $\C{D}_i$ is drawn from the joint distribution $p_i(x, y)$ over $\C{X} \times \C{Y}$ with the marginals given by $p_i(x)$ and $p_i(y)$. 

% \vspace{-1em}
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/gm_CPMAML.jpeg}
    \caption{A graphical model representing our hierarchical Bayes framework with task-agnostic meta-parameters $\theta$ and task-specific latent variables $z^x_i$, $z^y_i$ which influence the marginal $p_i(x)$ and conditional $p_i(y|x)$ distributions respectively. The dotted lines denote the variational approximations introduced over the true posteriors. 
    % The objective remains to learn variational parameters that suitably maximize the likelihood of the observed variables (shaded).
    }
    \label{fig:gm_CPMAML}
\end{figure}

The probabilistic model we consider in our work is summarized in Fig.~\ref{fig:gm_CPMAML}. Without making any assumptions on the nature of $p_i(x, y)$, we assume the existence of meta-parameters $\theta$ that govern the common structure shared across the set of joint distributions $\{p_{i}(x,y)\}_{i=1}^{n}$.
% as opposed to just the conditional $p_{i}(y)$ as done by \am{add citations}. 
Within each task the generative model for the input $x^{(i)}$ involves a random variable $z^{x}_{i}$ which we shall refer to as the latent factors of the covariate distribution.
Also, each task has an additional latent variable $z^{y}_{i}$ which plays a role in the generative model for the response variable $y^{(i)}$ given the input $x^{(i)}$.
In most settings, a naive assumption of independence is made over the latent factors $z^{x}_{i}$ and $z^{y}_{i}$. On the other hand, we refrain from making such assumptions and instead exploit the information present in the covariates $\{\V{x}_j^{(i)}\}_{j=1}^{m}$ to better infer the posterior over the latent variable $z^{y}_i$ which influences the conditional $p_i(y|x)$.
% The meta-parameter is given by the random variable $\theta$ and the parameters of the conditional $p_{i}(y)$ and the marginal $p_{i}(x)$ are given by $z_{y}^{(i)}$ and $z_{x}^{(i)}$ respectively. Most works \am{add citations here} assume that the posterior $p_{i}(z^{x}, \beta | \C{D})$ can be factored into $p_{\C{T}}(\phi | \C{D})$ and $p_{i}(\beta | \C{D})$. In this work we refrain from making such assumptions and instead propose a solution that exploits the meta-relationship between the posterior over the task specific parameters $p_{\C{T}}(\phi|\beta, \C{D})$ and the posterior over the parameters of the covariate distribution  $p_{\C{T}}(\beta | \C{D})$.

% Assume we observe data from N tasks, where the $i^{th}$ task consists of data $\C{D}_i$, each containing M datapoints as $\C{D}_i = \{(x_{j}^{(i)}, y_{j}^{(i)})\}_{j=1}^{M}$. As given in figure \ref{fig:gm_CPMAML}, we assume global latent variable $\theta$ and task-specific latent variable $(\beta_i,\phi_i)$ for all $i \in \{1,2,\dots N\}$. 
\subsection{Formal Derivations}
\label{subsec:formal_derivations}
In this section, we derive a lower bound for the likelihood of the observed data $\{\C{D}_i^{S}\}_{i=1}^{n}$ using hierarchical variational inference. This gives us the meta-learning objective that can be optimized using standard gradient-based approaches.
\begin{align}
    \label{eq:deriv-1}
    \log &\,\, p(\{ \C{D}_i^{S} \}_{i=1}^n) = \log \int_\theta p(\{\C{D}_i^{S}\}_{i=1}^n | \theta) p(\theta) \; d\theta   \\
    & \geq \R{E}_{q(\theta; \beta)} \left[ \sum_{i=1}^{n}\log p(D_i^{S} | \theta) \right] - \textsc{kl}(q(\theta; \beta)  || p(\theta)) \nonumber
\end{align}
In the above equation, the distribution $q(\theta; \beta)$ is a variational approximation (with parameters $\beta$) for the true posterior over the meta-parameter $\theta$. For the derivations henceforth we shall drop the notations $i$ and $S$ when understood from context. The log-likelihood of the dataset $\C{D}_i$ given by $p(\C{D}_i|\theta)$, can be written as an integral over the factors $p(\C{D}_i|z^x_{i}, z^{y}_{i})$, $p(z^{y}_{i}|z^{x}_{i}, \theta)$ and  $p(z^{x}_{i} | \theta)$.
\begin{align}
   p(\C{D}_i|\theta) \hspace{-0.1em} = \hspace{-0.1em} \int_{z^x_i} \hspace{-0.3em}\int_{z^y_i} p(\C{D}|z^x_i, z^y_i) p(z^y_i|z^x_i, \theta) p(z^x_i|\theta)\;\;  dz^y_i dz^x_i \nonumber
\end{align}
To lower bound the log of the above objective we introduce two variational approximations (i) $q(z^x_i; \kappa_i)$ with parameters $\kappa_i$ for the true posterior $p(z^x_i | \{\V{x}_j^{(i)}\}_{j=1}^{m'})$ and (ii) $q(z^y_i; \lambda_i)$  with parameters $\lambda_i$ for the true posterior $p(z^y_i | z^x_i, \C{D}_i^{S})$.
\begin{align}
     \log p(\C{D}_i|\theta) & \hspace{-0.2em} \geq  \hspace{-0.2em} \R{E}_{q(z^x_i;\kappa_i)} \hspace{-0.4em} \left[ \log \int p(\C{D}_i | z^x_i, z^y_i) p(z^y_i | z^x_i, \theta)  dz^y_i \right] \nonumber \\  
     & - \textsc{kl}(q(z^x_i;\kappa_i) || p(z^x_i|\theta))
     \label{eq:deriv-elbo-zx}
\end{align}
% \begin{align}
%       \beta, \theta) p(\beta|\theta) \; d\phi d\beta \\  \nonumber
%       \geq  \R{E}_{q(\beta;\kappa_i)} & \left[ \log \int_{\phi} p(\C{D}_i | \phi, \beta) p(\phi | \beta, \theta) d\phi \right] \\ \nonumber
%   &- \textsc{kl}(q(\beta;\kappa_i)||p(\beta|\theta)) 
% \end{align}
Since $z^x_i$ is the latent factor in the generative model for $x^{(i)}$ and $z^{y}_{i}$ is the corresponding latent variable for $y^{(i)}$, we arrive at the independence: $\V{y}_{j}^{(i)} \perp z^x_i | z^y_i, \V{x}_{j}^{(i)}$ and $\V{x}_{j}^{(i)} \perp z^y_i| z^x_i$. Based on this, we finally arrive at the following Evidence Lower Bound (\textsc{elbo}) for $\log p(\C{D}_i | \theta)$ which we shall refer to as $\C{L}_{\C{D}_i}(\kappa_i, \lambda_i, \theta)$. 
% \begin{align}
%   & \log p(\C{D}_i | \theta) = \log \int_{\beta} \int_{\phi} p(\C{D}_i | \phi, \beta) p(\phi | \beta, \theta) p(\beta|\theta) \; d\phi d\beta \\
%   & \geq  \R{E}_{q(\beta;\kappa_i)} \left[ \log \int_{\phi} p(\C{D}_i | \phi, \beta) p(\phi | \beta, \theta) d\phi \right] - \textsc{kl}(q(\beta;\kappa_i)||p(\beta|\theta))
% \end{align}
% \begin{align}
%     \log p(\C{D}_i | \theta) \geq \C{L}_{\C{D}_i}(\kappa_i, \lambda_i, \theta)
% \end{align}
\begin{align}
\label{eq:deriv-elbo-zy}
   & \C{L}_{\C{D}_i} (\kappa_i, \lambda_i, \theta) = \R{E}_{q(z^x_i;\kappa_i)}\left[  \sum_{j=1}^{m'} \log p(\V{x}_j^{(i)} | z^x_i) \right]  \\
    - & \textsc{kl}(q(z^x_i;\kappa_i)  ||  p(z^x_i|\theta)) +  \R{E}_{q(z^x_i;\kappa_i)} \;  \C{L}_{\C{D}_i}'(z^x_i, \lambda_i, \theta) \nonumber \\
    \label{eq:deriv-elbo-zy-2}
    & \C{L}_{\C{D}_i}'(z^x_i, \lambda_i, \theta) =   \R{E}_{q(z^y_i;\lambda_i)} 
    \left[ \sum_{j=1}^{m'} \log p(\V{y}_j^{(i)} | \V{x}_j^{(i)}, z^y_i) \right]  \nonumber \\  
     & \quad\quad\quad\quad\quad\quad-  \textsc{kl}(q(z^y_i;\lambda_i)||p(z^y_i|z^x_i, \theta))  
\end{align}
    % & + \R{E}_{q(\beta;\kappa_i)}\left[  \sum_{j=1}^{M} \log p(\V{x}_j^{(i)} | \beta) \right] - \textsc{kl}(q(\beta;\kappa_i)||p(\beta|\theta)

Therefore, the \textsc{elbo} on the likelihood of the dataset for $i^{th}$ task is a function of the task-specific variational parameters $\kappa_i, \lambda_i$ and the variational meta-parameter $\beta$. For each task, the optimal variational parameters that approximate the true posteriors are distinct. Hence, $\kappa_i, \lambda_i$ need to be adapted for each task individually. 
% Following popular work in amortized variational inference \cite{ravi2018amortized}, the adaptation is done using standard gradient ascent. 
Given $ \C{L}_{\C{D}_i} (\kappa_i, \lambda_i, \theta)$ we can re-write the lower bound in Eq.~\ref{eq:deriv-1} as:
\begin{align}
\label{eq:final-elbo}
& \quad\quad\quad\quad \quad\log \,\, p(\{ \C{D}_i^{(S)} \}_{i=1}^n) \geq \C{L}(\beta)   \\
& = \R{E}_{q(\theta; \beta)} \left[ \sum_{i=1}^{n} \C{L}_{\C{D}_i}(\kappa_i, \lambda_i, \theta)  \right] - \textsc{kl}(q(\theta; \beta)  || p(\theta)) \nonumber
\end{align}

\subsection{Algorithm}
\label{subsec:algorithm}
% \sd{for the second loss term, first assumption is  $q(z^y_i|\lambda_i) = \delta(\lambda_i)$. Further, $z^y_i$ represent the parameters of neural network that take in x and spits out y. Therefore, maximizing first term for $\lambda_i^*$ is same as SGD with some loss, For the second term, which act as regularizer to this optimal $\lambda_i$. Instead of explicitly writing the \textsc{kl} term, we regulairize by choosing the initialization for $\lambda_i$ SGD. For most prior work, this initialization is contained in $\theta$ itself. However, here we make the initialization to depend on $z^x_i$. Since, its again difficult to explicitly represent this dependance we use a neural network with parameters $\theta^' \in \theta$ shared task-agnostic that takes in input as $z^x_i$ and spits out the initialization. }

% \sd{Assume that $q(z^x_i)=N(u_k, s_k)$ then assume that $p(z^x_i|\theta)$ is independent of $\theta$ and is N(0,1) Now we know that optimal $k^*$ for the task is function of the dataset $D^s$. Let's assume that this dependence is given by a neural network with parameters $\theta$ write $u = u_\theta(D_s)$ and similarly sigma. Use reparameterization trick to evaluate both the expectations. This gives me $L(\theta, k^*, \lambda_i^*)$. Now to optimize for $\theta$ in the outer loop, the gradient is simple as for the first two terms are same as VAE therefore we do SGD on the reconstruction error. The parameters of the network that gives initalization from the $z^x_i$ can be updated using the loss backpropogated from y loss. We use $D_q$ for this meta-parameter update.}

% \am{talk abt opt objective from top down. meta-level then inner loop, then strip down the inner loop with the assumptions we make.}


The primary aim of any meta-learning algorithm is to optimize for the meta-parameter $\theta$ given the datasets $\{\C{D}_i\}_{i=1}^{n}$ from the corresponding sequence of tasks. This is generally a two step process where step-I involves identifying the optimal task-specific parameters using $\theta$ and the support set $\C{D}_i^{S}$. In step-II, based on the task-specific adapted parameters from step-I the meta-parameter $\theta$ is optimized over the query set $\C{D}_i^{Q}$. Within our framework, since both the meta-parameter $\theta$ and the task-specific parameters $z^x_i, z^y_i$ are Bayesian random variables with variational parameters given by $\beta, \lambda_i, \kappa_i$ respectively, we instead define an algorithm to optimize the \textsc{elbo} in Eq.~\ref{eq:final-elbo}.
\begin{align}
    \label{eq:outer-loop}
    \beta^* &= \arg\min\limits_{\beta} \;  -\C{L}(\beta) \\
    &= \arg\min\limits_{\beta} \;  -\R{E}_{q(\theta; \beta)} \sum\limits_{i=1}^n  \C{L}_{\C{D}_i^{Q}}(\kappa_i^*, \lambda_i^*, \theta) \nonumber \\
    & \quad \quad \quad \quad \quad \quad \quad \quad  + \textsc{kl}(q(\theta; \beta)  || p(\theta)) \nonumber  \\
    % \hat{\kappa_i}^{(i)}\C{L}(\beta, \hat{\kappa_i}^{(i)}, \hat{\lambda_i}^{(i)}) \\
    \label{eq:inner-loop}
    &\kappa_i^* , \lambda_i^* = \arg\min\limits_{\kappa_i, \lambda_i} \; -\R{E}_{q(\theta; \beta)} \C{L}_{\C{D}_i^{S}}(\kappa_i, \lambda_i, \theta)
\end{align}
 In order to optimize the objectives in Eqs.~\ref{eq:outer-loop},~\ref{eq:inner-loop}  we introduce certain simplifying assumptions over each of the variational approximations in Sec.~\ref{subsec:formal_derivations}. \footnote{We note that the assumptions we consider are merely to induce a computationally feasible meta-learner and the theory involving a meta-distribution over covariates (in Sec.~\ref{subsec:formal_derivations}) is barely undermined by it.}
% Based on these we re-write the \textsc{elbo} in Eq.~\ref{eq:elbo} which would in turn result in a meta-optimization algorithm that uses the structure uses the covariate distribution over tasks.
\begin{assumption}
\label{assm:theta}
The variational approximation $q(\theta; \beta)$ follows a $\delta-$distribution given by $\delta_{\beta}$ and the prior $p(\theta)$ is given by $\C{N}(\V{0}, \V{I})$. We note that the assumptions taken are effective in arriving at a computationally feasible algorithm and are
\end{assumption}
\begin{assumption}
\label{assm:z}
The variational approximation $q(z^y_i; \kappa_i)$ follows a normal distribution with mean, diagonal co-variance matrix given by $\kappa_i^*= (\gamma_\mu(\C{D}_i^{S}; \beta), \gamma_\sigma^2(\C{D}_i^{S}; \beta))$. The prior $p(z^x_i|\theta)$ is taken as $\C{N}(\V{0}, \V{I})$. On the other hand, the distribution $q(z^x_i; \lambda_i)$ is given by a $\delta-$distribution: $\delta_{\lambda_i}$. 
\end{assumption}
% mean $\mu_{\kappa_i}(\C{D}_i^{(S)})$ and variance $\sigma^2_{\kappa_i}(\C{D}_i^{(S)})$ 
% \begin{assumption}
% Also, the variational parameters of $q(z^y_i; \kappa_i)$ are shared across tasks and can be considered as part of the meta-parameter $\theta$.
% \end{assumption}

Using Assms.~\ref{assm:theta},~\ref{assm:z} the Eqs.~\ref{eq:outer-loop},~\ref{eq:inner-loop} can be re-written as a two layer log-likelihood objective with an $l_2$ regularization term.
\begin{align}
\label{eq:outer-rewrite}
\beta^* &= \arg\min_{\beta} \;  -\sum_{i=1}^{n} \C{L}_{\C{D}_i^Q}(\kappa_i^*, \lambda_i^*, \beta) + \frac{1}{2} \|\beta\|_2^2 \\
\label{eq:inner-rewrite}
\lambda_i^* &=  \arg\min\limits_{\lambda_i} \; -\C{L}_{\C{D}_i^{S}}(\kappa_i^*, \lambda_i, \beta)\\
\kappa_i^* &= (\kappa_i^*(\mu), \kappa_i^*(\sigma)) = (\gamma_\mu(\C{D}_i^{S}; \beta), \gamma_\sigma(\C{D}_i^{S}; \beta))
\end{align}

To be concrete, the task-specific random variable $z^y_i$ represents the parameters of the neural network for the $i^{th}$ task, that takes as input $\V{x}_j^{(i)}$ and outputs a prediction $\V{\hat{y}}_j^{(i)}$. On the other hand, as stated previously $z^x_i$ represents the latent variable for the covariate distribution $p_i(x)$. Furthermore, the optimal variational parameters for the distribution $q(z_x^i;\kappa_i)$ is given by $\kappa_i^*$ which consists of the mean $\gamma_\mu(\C{D}_i^{S}; \beta)$ and std. deviation $\gamma_\sigma(\C{D}_i^{S}; \beta)$ of a normal distribution. Here, $\gamma_\mu(\cdot, \beta), \gamma_\sigma(\cdot, \beta)$ represent neural networks which take as input the support set $\C{D}_i^{S}$ and output $\kappa_i^*$. It is important to note that even though the parameters of $\gamma_\mu, \gamma_\sigma$ are task-agnostic, the variational parameter $\kappa_i^*$ is still different for each task and is determined using the covariates in $\C{D}_i^{S}$.


Having identified $\kappa_i^*$ we now describe the optimization algorithm for $\lambda_i$ in Eq.~\ref{eq:inner-rewrite}. Notice that to obtain $\lambda_i^*$ it is sufficient to only minimize the objective $-\R{E}_{q(z_i^x; \kappa^*)}\C{L}_{\C{D}_i}'(z_i^x, \lambda_i, \beta)$. In Eq.~\ref{eq:deriv-elbo-zy-2} the \textsc{kl} term acts as a regularizer in the optimization objective for $\lambda_i$. 
Since the most common algorithm for optimization is Stochastic Gradient Descent (\textsc{sgd}) many meta-learning algorithms avoid the \textsc{kl} term by choosing a regularization specific to \textsc{sgd}. 
In most works \cite{ravi2018amortized, finn2018probabilistic, kim2018bayesian}, the \textsc{kl} term is a function of only the meta-parameter $\theta$ (or $\beta$ given Assm.~\ref{assm:theta}). Hence the regularization is induced by letting the initialization for the optimization of $\lambda_i$ (given by $\lambda_i^{(0)}$) be determined by $\beta$.
In our framework, we realize that the \textsc{kl} term is a function of both $\beta$ and the latent variable $z^x_i$ for the task specific covariate distribution. 
Hence we model the initialization  $\lambda_i^{(0)}$ using a neural-network whose parameters are subsumed in $\beta$ and thus without loss of expressivity $\lambda_{i}^{(0)}=f_\beta(z^x_i)$ . 
Thus, the optimal parameters of the variational approximation ($\lambda_i^*$) would be given by performing $K$ steps of \textsc{sgd} on the \textsc{mle} objective in Eq.~\ref{eq:deriv-elbo-zy-2} with the initialization given by $f_\beta(z^x_i)$.
\begin{align}
    \label{eq:deriv-elbo-zy-2-rewrite}
    \lambda_i^{*} = \R{E}_{q(z_i^x; \kappa_i^*)} \; & \textsc{sgd}\footnotemark(l_{\C{D}_i}(\lambda_i), \lambda_i^{(0)} = f_\beta(z^x_i), K) \\
    l_{\C{D}_i}(\lambda_i) &=  -
   \sum_{j=1}^{m'} \log p(\V{y}_j^{(i)} | \V{x}_j^{(i)}, \lambda_i) \nonumber
\end{align}

\footnotetext{$\textsc{sgd}(l(\lambda),\lambda^{(0)},K)$ is the parameter obtained by performing $K$ steps of \textsc{sgd} on the objective $l(\lambda)$ with initialization $\lambda^{(0)}$.}

The expectation in Eq~\ref{eq:deriv-elbo-zy-2-rewrite} is computed using monte-carlo approximation. We find that sampling a single value of $z_i^x \sim q(z_i^x; \kappa_i^*)$ is sufficient to optimize for $\lambda_i$.  





% \footnotetext{Note the re-parameterization trick.}

\begin{algorithm}[H]
\caption{Meta-training Algorithm}
\begin{algorithmic}
 \STATE Given: $n$ datasets: $\{\C{D}_i^S, \C{D}_i^Q\}_{i=1}^{n}$, learning rates: $\eta_0, \eta_1$, number of update steps: $K$.  \\
%  \STATE Initialize $\theta=\{\mu_\theta, \sigma^2_{\theta}, \lambda_i^{(init)}_{\theta} \}$\\
 \STATE $p(\theta), p(z^x_i|\theta) \gets \C{N}(\V{0}, \V{I})$     
 \FOR{i=1 to n}
        % \STATE $\mu^{(0)}_{\kappa_i} \gets \mu_\theta ; \sigma^{2(0)}_{\kappa_i} \gets \sigma^2_\theta $ 
        \STATE $\kappa_i^*(\mu), \kappa_i^*(\sigma) \gets \gamma_\mu(\C{D}_i^{S};\beta), \gamma_\sigma(\C{D}_i^{S};\beta)$ \\
        \STATE $\lambda_i^{(0)} = f_\beta(\kappa_i^*(\mu) + \epsilon \circ \kappa_i^*(\sigma))$; $\;\;\;\epsilon \sim  \C{N}(\V{0}, \V{I})$   \\
        % \STATE $\lambda_i^{(0)}$
        % \STATE $z_x^i \gets \tilde{z}_x^i$ \\
        \FOR{t=0 to K-1}
            % \STATE $\kappa_i^{(j)} \gets \{\mu_\kappa_i^{(j)}, \sigma_\kappa_i^{(j)}\}$
            \STATE $\lambda_i^{(t+1)} \gets  \lambda_i^{(t)} - \eta_0 \nabla_{\lambda_i^{(t)}} \sum\limits_{j=1}^{m'} \log p(\V{y}_j^{(i)} | \lambda_i^{(t)} , \V{x}_j^{(i)})  $ \\
            % \STATE ${\sigma^2_\kappa_i}^{(j+1)} \gets  {\sigma^2_\kappa_i}^{(j)} - \alpha \nabla_{\sigma_\kappa_i^{2(j)}} \C{L}_{\C{D}_i^{(S)}}(\kappa_i^{(j)} , \lambda_i_\theta^{(init)}, \theta)$
        \ENDFOR
        % \STATE $z_x^i \gets \tilde{z}_x^i$ \\
        \STATE $\lambda_i^*  \gets  \lambda_i^{(K)}$ 
        
        % \STATE $\lambda_i^*  \gets  \lambda_i^{(K)}$ 
        
        
        % \FOR{j=0 to K-1}
        %     \STATE $\lambda_i^{(j+1)} \gets  \lambda_i^{(j)} - \alpha \nabla_{\lambda_i^{(j)}} \C{L}_{\C{D}_i^{(S)}}(\kappa_i^{(K)}, \lambda_i^{(j)}, \theta)$
        % \ENDFOR
        
        % \STATE $q(\theta) = \C{I}\{\mu = \mu_\theta \} \cdot \C{I}\{\sigma^2 = \sigma^2_\theta \} \cdot \C{I}\{ \lambda_i^{(init)} = \lambda_i^{(init)}_\theta \}$
        
        \STATE $\beta \gets  \beta - \eta_1 \nabla_{\beta} \left[ \sum\limits_{i=1}^{n} \C{L}_{\C{D}_i^Q}(\kappa_i^*, \lambda_i^*, \beta) - \frac{1}{2} \|\beta\|_2^2\right]$
        
        % \STATE $\sigma^2_\theta \gets  \sigma^2_\theta - \beta \nabla_{\sigma^2_\theta} [  \C{L}_{\C{D}_i}(\kappa_i^{(K)}, \lambda_i^{(K)}, \theta) + \frac{1}{M} \textsc{kl} (q(\theta) || p(\theta)) ]$
        % \STATE $\lambda_i^{(init)}_\theta \gets  \lambda_i^{(init)}_\theta - \beta \nabla_{\lambda_i^{(init)}_\theta} [ \C{L}_{\C{D}_i}(\kappa_i^{(K)}, \lambda_i^{(K)}, \theta) + \frac{1}{M} \textsc{kl} (q(\theta) || p(\theta)) ]$
 \ENDFOR
 \end{algorithmic}
 \label{alg:train}
\end{algorithm}



Finally, we note that the meta-parameter $\beta$ constitutes the parameters of the network $f_\beta$ which determines the initialization $\lambda_i^{(0)}$ as well as the parameters of $\gamma_\mu(\cdot; \cdot), \gamma_\sigma(\cdot; \cdot)$ which output $\kappa_i^*$.  
Thus, $\beta$ is optimized to jointly maximize the likelihood of the covariates of a sequence of tasks as well as for learning to choose covariate dependent initializations suitable for few-shot adaptation.
For the optimization objective in Eq.~\ref{eq:outer-rewrite}, we use the standard re-parameterization trick ($2^{nd}$ step of the outer \textit{for-loop} in Algorithm~\ref{alg:train}) commonly used in Variational Auto-Encoders (\textsc{vae}s). This is done so as to be able to differentiate through the expectation over $q(z_i^x; \kappa_i^*)$ in Eqs.~\ref{eq:deriv-elbo-zy}, ~\ref{eq:deriv-elbo-zy-2-rewrite}. The step-by-step procedure for the meta-training and meta-testing phases are given by Algorithm~\ref{alg:train} and Algorithm~\ref{alg:test} respectively.

% Based on Assm.~\ref{assm:z}, we can avoid the \textsc{kl} term: $\textsc{kl}(q(z^x_i;\kappa_i) || p(z^x_i|\theta))$ present in Eq.~\ref{eq:deriv-elbo-zx} since by further assuming $ p(z^x_i|\theta)$ to be. we can re-write the term $\C{L}_{\C{D}_i}(\kappa_i, \lambda_i, \hat{\beta})$ in Eq.~\ref{eq:final-elbo-rewrite}. 
% \begin{align}
% \label{eq:elbo-rewrite}
% \C{L}(\kappa_i, \lambda_i, \hat{\beta})  = \sum_{i=1}^{n} \C{L}_{\C{D}_i}(\kappa_i, \lambda_i, \hat{\beta}) - \frac{1}{2} \|\hat{\beta}\|_2^2 
% \end{align}







% \am{specific instantiation here.}

% Having introduced the 

% In this section, we formalize our algorithm. Our algorithm for meta-training and testing is inspired by that in \cite{ravi2018amortized}. The key difference lies in the learning procedure for the variational parameters corresponding to the latent variable $\beta$ that we introduced in our work. \\
% As common in many meta-learning approaches, the optimizations takes place in two nested loops. The inner loop updates the task-specific parameters ($\kappa_i, \lambda_i$ here), while the outer loop updates global meta-parameters ($\theta$ here). As we briefly described in the previous section, we can decompose our meta-parameters into two parts. $\theta = ((\mu_\theta, \sigma^2_\theta), \lambda_i^{(init)}_\theta)$. The first part corresponds to both the initialization for the task specific parameters $\kappa_i$, as well as define the prior $p(\beta|\theta)$, which we assume normal for our specific formulation. Further, we take $\lambda_i^{(init)}_\theta$ to explicitly represent the initial value for $\lambda_i$ which is used when we update our task-specific parameters in the inner-loop. \\
% In the task specific adaptation, we update the variational parameters using standard gradient ascent. Let $\kappa_i_{\C{D}_i}^* =SGD^{(K)}(\kappa_i^{(init)}, \lambda_i^{(init)}, \theta)$ represent the variational parameters for the distribution $q(\beta;\kappa_i)$ after $K$ steps of gradient ascent on the objective $\C{L}_{\C{D}_i}(\kappa_i, \lambda_i, \theta)$. Note that, we could have chosen $\kappa_i^{(init)}, \lambda_i^{(init)}$ arbitrarily, but we use $\theta$ as initialization for it has been shown that it has many performance benefits. This can be attributed to the fact that $\theta$ is shared across all tasks and updated to suit each one of them in the outer-loop update. Therefore, these initializations are close to optimal and even a few steps of gradient updates lead us to the optimal values. Similarly, the variational parameters for the distribution $q(\phi;\lambda_i)$ after $K$ gradient steps is given by $\lambda_i_{\C{D}_i}^* =SGD^{(K)}(\kappa_i_{\C{D}_i}^*, \lambda_i^{(init)}, \theta)$. Note that we carefully defined our gradient descent to have stepwise updates, where we first update the parameters $\kappa_i$ using $\lambda_i^{(init)}$. We hypothesise that due to meta-learning (in the outer-loop), the initialization of $\lambda_i$ will be close to the optimum $\lambda_i^*$ for this task. Then we use the optimal $\kappa_i^*$ to optimize for $\lambda_i$. We chose this method over joint learning primarily to simplify learning given we have only few examples. Also, this helps us to encapsulate semi-supervised learning objectives in our framework as mentioned in the next section. \\

% the initialization of which is encapsulated in the task-agnostic parameter $\theta$. Therefore, $\theta$ plays a dual role of representing the parameters used to model prior distributions $p(\beta|\theta)$ and $p(\phi|\beta,\theta)$ as well as initialization for variational parameters. More details regarding task-specific adaptation can be found in the following section.


 


% We assume a meta-distribution over $p_{\C{T}}(x,y)$ (instead of  $p(y)$ and hence we define our graphical model (as shown in \ref{fig:gm_CPMAML}) to consist of two task specific latent variables $\beta$, $\phi$ which share a common task-agnostic prior $\theta$. $\beta_i$ for each task is used to model the covariates $x_i$ for that task and $\phi_i$ is used to model $y_i| x_i$.

% To include the proposed dependence between covariate distribution and $p(y)$, we add another edge (dependence relation) from $\beta_i$ to $\phi_i$ for each task. Although, for classification and regression, we are only interested in knowing $P(y)$ (and hence only the latent variables $\phi$) for an unseen-task, such a formulation helps to improve our estimates by leveraging the information from covariates during meta-training. As we will show with a concrete example, we can use the learnt covariate distribution to adapt various versions of existing semi-supervised learning in our framework even without any need of unlabelled data. The relation between semi-supervised learning and our approach is that former uses unlabelled data to model distribution $p(x)$ for a particular task while we extract information about $p(x)$ from multiple-tasks and adapt it to the particular task without the need of the data. Both the methods, use this information to improve the estimates for $y$ in a similar manner. \\

% In this section, we analyse the probabilistic MAML framework as defined in \cite{finn2018probabilistic} for covariate shift problem as discussed above. In this framework, we learn a prior over the parameters for the regression function ($f_\theta : \C{X} \rightarrow \C{Y} $ as defined above) during meta-training. Then for each task, we compute the posterior distribution of these parameters using the training samples as well as the learned prior. This framework learns and encodes the information related to the meta-distribution into the prior. Although, the meta-distribution exists over the joint distribution of $p(x,y)$ (ie both $p(x)$ and $p(y)$) but here we restrict the prior to only $p(y)$. We believe that we can similarly learn a prior over the distribution of the covariates and use it in task specific posterior computation. Also, if we are given large number of unlabelled samples for each task, then the error in the computation of such a prior reduces.

% However, our approach relies on the existence of Bayesian random-design regression methods in the inner loop which can use the prior over the covariates to reduce the risk in computation of the response function ($m(x) = E(y)$). We can formalize this critical question as the following. Bayesian regression problem can be defined as- Let $m(\V{x}) = E(y|\V{x})$ be parameterized by $\phi$. The goal is to compute the posterior distribution of $\phi$ given iid samples $ \{(\V{x}_i, y_i)_{i=1}^{K}\}$ from the joint distribution of $p(\V{x},y)$ and prior $p(\phi)$. Now suppose, in addition to the prior on the parameters $\phi$, we are also given the distribution $p(\V{x})$, can we use it to improve our posterior distribution such that it reduces the true risk of the regression estimator $\hat{\phi}$. If we can answer positively to the above question, then we can formulate our apporach as follows.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/gm_MAML.png}
%     \caption{Graphical models for meta-learning framework. Dotted lines denote variational approximations. (a) Original setup where inference parameters are learned separately for each episode (b) Standard amortized variational inference scheme (c) Amortized variational inference scheme specific to MAML with train (S) and test (Q).}
%     \label{fig:gm_MAML}
% \end{figure}

% \subsubsection{Approach}


 


% In the optimization for $\kappa_i$ we adopt posterior regularization. This gives rise to the regularized bayes framework where instead of maximizing over the objective 



% \subsection{Approach}
% \label{subsec:algorithm}

% \begin{center}
% \begin{align}
%     \lambda_i \gets \lambda_i
% \end{align}
% \end{center}




% \begin{align}
%     \C{L}_{\C{T}}(\V{z}) = \B{E}_{x}[\C{L}(f_\phi(\V{z}, \V{x})] = \int_\beta \int_x  \C{L}(f_\phi(z), \V{x}) p(\V{x}|\beta) p(\beta) d\V{x} d\beta 
% \end{align}

% Variational Approximation:
% $$
% \theta = \{\kappa_i, \}
% $$

% $$
% L(x) = \|x - f_\eta(\kappa_i)\|_2^2
% $$

% \begin{align}
%     \C{L}_{\C{T}}(\, \theta) = \B{E}_{\beta \sim q(\beta|z,\theta)} \left[\int_x  \C{L}(f_\phi(\V{z}, \V{x}) p(\V{x}|\beta) d\V{x} \right]  - \textsc{kl}(q_\C{T}(\beta|\V{z},\V{\theta}) || p(\beta))
% \end{align}

% \begin{align}
%     q_{\C{T}}(\beta|\V{z},\V{\theta}) = \delta(\theta_x - \nabla_\theta \C{L}_{\C{T}}(\V{z}, \theta))
% \end{align}



% \begin{algorithm}[H]
% \caption{Meta-Training Algorithm}
% \begin{algorithmic}
%  \STATE Given: Tasks $\C{T}_1 \dots \C{T}_N$ with ${\V{z}_i}^{\mathrm{tr}}, {\V{z}_i}^{\mathrm{te}}$ labeled samples for task $\C{T}_i$ \\
%  \STATE Given: Learning rates  $\alpha, \beta$ \\
%  \STATE Given: Initial parameters $\theta_0, \phi_0$ for algorithm $\C{A}(\theta, \phi)$. 
%  \FOR{i=1 to N}
%         \STATE $\phi^{i}_{0} \gets \phi_i$
%         \STATE Estimate $q(\beta|\V{x}_i, \theta) = \C{N}(g^{\mu}_\theta(\V{x}_i), g^{\sigma}_\theta(\V{x}_i))$\\
%         \FOR{j=1 to n}
%             \STATE $\phi^{i}_{j+1} \gets \phi^{i}_{j} - \alpha \nabla_\phi \C{L}_{\C{T}_i}({\V{z}_{i,j}}^{\mathrm{tr}}, \theta_{i})$
%         \ENDFOR
%         \STATE $\phi_{i} \gets \phi_{i-1} - \beta \nabla_\phi \C{L}_{\C{T}_i}({\V{z}_i}^{\mathrm{te}}, \theta_{i})$
%         \STATE $\theta_{i} \gets \theta_{i-1} - \beta \nabla_\theta \C{L}_{\C{T}_i}({\V{z}_i}^{\mathrm{te}}, \theta_{i})$
%  \ENDFOR
%  \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{Inference Algorithm: Meta-testing}
% \begin{algorithmic}
% %  \STATE Given: Tasks $\C{T}_1 \dots \C{T}_N$ with ${\V{z}_i}^{\mathrm{tr}}, {\V{z}_i}^{\mathrm{te}}$ labeled samples for task $\C{T}_i$ \\
%  \STATE Given: $M$ Tasks $\C{D}_1, \C{D}_2 \dots \C{D}_M$ \\
%  \STATE Given: Learning rates  $\alpha, \beta$ \\
%  \STATE Initialize $\theta=\{\mu_\theta, \theta_{y}\}$ for algorithm $\C{A}(\theta)$. 
%  \FOR{i=1 to N}
%         \STATE $\phi^{i}_{0} \gets \theta_{y}$
%         \STATE $\beta^{i}_{0} \gets \theta_{x}$
%         \FOR{j=1 to n}
%             \STATE $\beta^{i}_{j+1} \gets \beta^{i}_{j} - \alpha \nabla_\beta () \C{L}_{\C{T}_i}({\V{z}_{i,j}}^{\mathrm{tr}}, \theta_{i})$
%         \ENDFOR
%         \STATE Estimate $q(\beta|\V{x}_i, \theta) = \delta()$\\
%         \FOR{j=1 to n}
%             \STATE $\phi^{i}_{j+1} \gets \phi^{i}_{j} - \alpha \nabla_\phi \C{L}_{\C{T}_i}({\V{z}_{i,j}}^{\mathrm{tr}}, \theta_{i})$
%         \ENDFOR
%         \STATE $\phi_{i} \gets \phi_{i-1} - \beta \nabla_\phi \C{L}_{\C{T}_i}({\V{z}_i}^{\mathrm{te}}, \theta_{i})$
%         \STATE $\theta_{i} \gets \theta_{i-1} - \beta \nabla_\theta \C{L}_{\C{T}_i}({\V{z}_i}^{\mathrm{te}}, \theta_{i})$
%  \ENDFOR
%  \end{algorithmic}
% \end{algorithm}








\begin{algorithm}[H]
\caption{Meta-testing Algorithm on test task $\C{T}$}
\begin{algorithmic}
 \STATE Given: dataset $\C{D}_{\C{T}} = \{\V{x}_j^{(\C{T})}, \V{y}_j^{(\C{T})}\}_{j=1}^{m}$, parameter: $\beta^*$, learning rate $\eta_0$, number of update steps: K.
 \STATE $\kappa_{\C{T}}^*(\mu), \kappa_{\C{T}}^*(\sigma) \gets \gamma_\mu(\C{D}_{\C{T}};\beta^*), \gamma_\sigma(\C{D}_{\C{T}};\beta^*)$ \\
        \STATE $\lambda_{\C{T}}^{(0)} = f_{\beta^*}(\kappa_{\C{T}}^*(\mu) + \epsilon \circ \kappa_{\C{T}}^*(\sigma))$; $\;\;\;\epsilon \sim  \C{N}(\V{0}, \V{I})$   \\
        \FOR{t=0 to K-1}
            \STATE $\lambda_{\C{T}}^{(t+1)} \gets  \lambda_{\C{T}}^{(t)} - \eta_0 \nabla_{\lambda_{\C{T}}^{(t)}} \sum\limits_{j=1}^{m} \log p(\V{y}_j^{(\C{T})} | \lambda_{\C{T}}^{(t)} , \V{x}_j^{(\C{T})})  $ \\
        \ENDFOR
        \STATE $\lambda_{\C{T}}^*  \gets  \lambda_{\C{T}}^{(K)}$ 
 \end{algorithmic}
 \label{alg:test}
\end{algorithm}


% \begin{algorithm}[H]
% \caption{Meta-Testing Algorithm$.}
% \begin{algorithmic}
%  \STATE Given: Test Dataset $\C{D} = \{\C{D}^{(S)}, \C{D}^{(Q)}\}$, Parameters $\theta = \{\mu_\theta, \sigma^2_{\theta}, \lambda_i^{INIT}_{\theta}\}$, Number of update steps K, Learning rate $\alpha$
%  \STATE $\mu^{(0)}_{\kappa_i} \gets \mu_\theta ; \sigma^{2(0)}_{\kappa_i} \gets \sigma^2_\theta $ 
        
%         \FOR{j=0 to K-1}
%             \STATE $\kappa_i^{(j)} \gets \{\mu_\kappa_i^{(j)}, \sigma_\kappa_i^{(j)}\}$
            
%             \STATE $\mu_\kappa_i^{(j+1)} \gets  \mu_\kappa_i^{(j)} - \alpha \nabla_{\mu_\kappa_i^{(j)}} \C{L}_{\C{D}^{(S)}}(\kappa_i^{(j)}, \lambda_i_\theta ^{(init)}, \theta)$
            
%             \STATE ${\sigma^2_\kappa_i}^{(j+1)} \gets  {\sigma^2_\kappa_i}^{(j)} - \alpha \nabla_{\sigma_\kappa_i^{2(j)}} \C{L}_{\C{D}^{(S)}}(\kappa_i^{(j)} , \lambda_i_\theta ^{(init)}, \theta)$
%         \ENDFOR
        
%         \STATE  $\kappa_i^{(K)} \gets \{\mu_\kappa_i^{(K)}, \sigma_\kappa_i^{2(K)}\}$
        
%         \STATE $\lambda_i^{(0)} \gets  \lambda_i^{(init)}_{\theta}$ 
        
%         \FOR{j=0 to K-1}
%             \STATE $\lambda_i^{(j+1)} \gets  \lambda_i^{(j)} - \alpha \nabla_{\lambda_i^{(j)}} \C{L}_{\C{D}^{(S)}}(\kappa_i^{(K)}, \lambda_i^{(j)}, \theta)$
%         \ENDFOR
%         % \STATE $q_\theta(\phi | \C{D}^{(S)}) = \delta(\phi;\lambda_i^{(K)})$
%         \STATE Evaluate $\C{D}^{(Q)}$ using $\R{E}_{q_{\theta}(\beta; \kappa_i^{K})} \left [ \R{E}_{q_{\theta}(\phi; \lambda_i^{K})} [p(\C{D}^{(Q)} | \phi, \beta)] \right]$
%  \end{algorithmic}
% \end{algorithm}
% We summarize the key points of difference between our work and the existing algorithms below:
% \begin{itemize}
%   \item We explicitly define meta-parameters to learn a prior on the covariate distribution of a task using covariates from multiple tasks.
%   \item We leverage the learnt prior to obtain the task-specific covariate distribution without the need of unlabelled samples.
%   \item For a particular task, the covariate distribution is then used to learn better estimators for model parameters corresponding to $p(y)$ by using existing semi-supervised learning methods and losses. 
%   \item The global meta-parameters are 
%   We use semi-supervised learning methods in the inner loop to directly benefit from the modelled task specific covariate distribution. This adds an additional loss computed from covariates to an existing learning objective.  
%   \item  We update the meta-parameters
% \end{itemize}


% The key difference in our approach to  \cite{ravi2018amortized} is the random variable $\beta$ which gives us the flexibility to model task specific covariate distribution. The uncertainity over the meta-parameter $\theta$ is now a function of the posterior over $\beta$ and $\phi$: or in other words it can account for the task specific response function and task specific covariate distribution. 


% \begin{align}
%     \arg \max\limits_{\mu_\theta, \nu_\theta, \psi} \log p(y_{tr} | \V{x}_{tr}, \mu_\theta, \nu_\theta) & \geq \B{E}_{\theta, \phi, \beta \sim q_\psi} \log p(y_{tr}|\V{x}_{tr}) + \log p(\phi|\theta)  \\
%     & + \log p(\beta|\theta) + \log p(\theta|\mu_\theta, \nu_\theta) + \C{H}(q_\psi(\phi|\theta, y_{tr}, \V{x}_{tr}))\\   
%     & + \C{H}(q_\psi(\beta|\theta, \V{x}_{tr})) +  \C{H}(q_\psi(\theta|\mu_\theta, \nu_\theta , \V{x}_{tr}))
% \end{align}

% By maximizing the lower bound  of the likelihood, we can compute the posterior distribution of the task specific parameters $\phi$ and $\beta$ for each task. These parameters help us model the uncertainity in measuring $p(y_{te}|\V{x}_{te})$ and $p(\V{x}_{te})$ respectively. Since, we have modelled the covariate distribution for each task, we plan to use semi-supervised learning methods for task-specific updates in the inner-loop. These semi-supervised methods leverage unlabelled data to give better estimators over their supervised counterparts. Here, we propose to leverage information about covariates from multiple tasks to benefit the estimates for our task-specific objective. Note that, we can achieve this even without requiring unlabelled data for each task since we explicitly model $p(x)$. 

% We will formalize the semi-supervised learning setting and the algorithm in later sections.

